Clustering-based redshift estimation: method and application to data

We present a data-driven method to infer the redshift distribution of an arbitrary dataset based on spatial cross-correlation with a reference population and we apply it to various datasets across the electromagnetic spectrum to show its potential and limitations. Our approach advocates the use of clustering measurements on all available scales, in contrast to previous works focusing only on linear scales. We also show how its accuracy can be enhanced by optimally sampling a dataset within its photometric space rather than applying the estimator globally. We show that the ultimate goal of this technique is to characterize the mapping between the space of photometric observables and redshift space as this characterization then allows us to infer the clustering-redshift p.d.f. of a single galaxy. We apply this technique to estimate the redshift distributions of luminous red galaxies and emission line galaxies from the SDSS, infrared sources from WISE and radio sources from FIRST. We show that consistent redshift distributions are found using both quasars and absorber systems as reference populations. This technique brings valuable information on the third dimension of astronomical datasets. It is widely applicable to a large range of extra-galactic surveys.

==> Dump_and_refs.tex <==





%If the redshift evolution of the bias $b_u(z)$ over $\Delta z$ is not negligible compared to the variation of $\phi_u(z)$, this method only allows us to estimate the product $\phi_u(z)\,b_u(z)$. Additional information from the auto-correlation of the unknown sample can be used to attempt breaking the degeneracy between these two quantities \citep[see for example][]{New:08}. 



When we depart from the ideal case considered above we can ask the question: how much error is induced by the lack of knowledge of $b_u(z)$?


%One reason for this is that the scale dependence of the bias is usually a slowly varying quantity. Moreover, 


The integrated dark matter correlation function $\bar w(z)$ can be estimated and the redshift-dependent bias of the reference sample can be obtained from a measurement of its auto-correlation function:


. The problem is fully solvable, up to some accuracy.

, up to some uncertainty given by the derivatives of the last three terms of Eq.~\ref{eq:w_full}, 


%over the interval $\Delta z$ we have
%\begin{equation}
%\frac{\rm d N_u}{\d z}(z_i) \propto
%{\bar w_{ur}(z)}
%\,
%\left( \frac{1}{\bar b_r(z)\,\bar w(z)} \right)~.
%\label{eq:estimator}
%\end{equation}


%%>>>> The more limited the interval $\Delta z$, the larger the variation of $\phi_u(z)$ and the smaller the variation of the other quantities.


%The integrated angular cross-correlation between the \emph{reference} sample and the \emph{unknown} sample can be written as
%\begin{equation}
%\frac{\rm d N_u}{\d z}(z_i) \propto
%\bar w_{ur}(z_i) \;
%%\frac{\rm d N_r}{\d z}
%\frac{1}{\bar b_u(z_i)\,\bar b_r(z_i)}\,
%%\bar w(z')
%\label{eq:w_full}
%\end{equation}
%%$\bar b_u^{\rm NL}$, 
%where $\bar w$ is the integrated dark matter correlation function (as defined in Eq.~\ref{eq:w_int}) and $\bar b_u(z)$ and $\bar b_r(z)$ are the corresponding integrated biases, defined as the square root of the ratios between the galaxy and dark matter correlation functions. 



%\bibitem[Phillipps \& Shanks(1987)]{1987MNRAS.227..115P} Phillipps, S., \& Shanks, T.\ 1987, \mnras, 227, 115 

%Benjamin J., van Waerbeke L., M ́enard B., Kilbinger M., 2010, MNRAS, 408, 1168

%\bibitem[Nikoloudakis et al.(2013)]{2013MNRAS.429.2032N} Nikoloudakis, N., Shanks, T., \& Sawangwit, U.\ 2013, \mnras, 429, 2032 

%% Roberts, O'Dell, Burbidge
%% at the time of Seldner \& Peebles



%
%A few authors have explored this avenue \citep[e.g.~]{New:08, Matt:10,Schu:10,Matt:12,McQ:13} and considered approaching the problem from a theoretical and global point of view. Here we take a different approach, taking into account its applicability to real-world datasets, emphasizing the interest of using small scale clustering information.

%If this correlation is significantly greater than random, it implies that the field $\delta F$ contains sources at redshift $z$ (we first ignore the small modulation possibly induced by gravitational magnification and discuss it in section~\ref{sec:lensing}). 


%We neglect the cross-correlation coefficient. Only affect things on small scales.
%


%, the normalization of the distribution given in  one needs to know 
%
%requires estimates of $\d{\rm N_u}/\d z$ at all redshifts of interest, the inferrence will depend on the redshift dependence of $b_u$ and $b_r$. 
%
%Here it is important to note that inferring the redshift distribution only requires the 
%needed as the redshift distribution is normalized through Eq.~\ref{eq:normalization}.



%(about $30 kpc$)The choice of the minimum angular scale is motivated 
%Most of the known redshifts originate from optical spectroscopic surveys. This motivates the choice of scale.


%Given that the large-scale structure of the Universe approaches that of a Gaussian random field, this quantity captures a significant fraction of the structure of the extragalactic sky. 


%leading to a much higher sensitivity and a wider applicability. 
%

%taking into account its applicability to real-world datasets, emphasizing the interest of using small scale clustering information.


%Let $n_i$ be the surface density of objects and $\delta n_i$ %be the corresponding density fluctuation $\delta_i=n_i/\langle n_i\rangle -1$, where $\langle n_i \rangle$ is the mean density. The index $i$ refers to the reference or unknown population. We introduce the normalized redshift distribution:
%\begin{equation}
%\phi_i(z) = 
%\left.
% \frac{\d^2 N_i}{\d z\d\Omega} 
%\; \middle /
%\right.
%{ \int{\d z\d\Omega}\, \frac{\d^2 N_i}{\d z\d\Omega} }
%\end{equation}
%where $\d^2 N_i/\d z\d \Omega$ is the number of objects per unit redshift and solid angle. 


%
%Previous studies making use of spatial correlations to infer redshift distributions focused only on large scales, on which the galaxy bias is sufficiently linear. For example, \citet{New:08} proposed a method to recover the redshift distribution of unknown populations, using measurements of the cross-correlation function on scales greater than a few Mpc. Here, instead we propose to measure the amount of clustering by integrating over all available scales. This approach allows us to significantly increase the signal-to-noise ratio (S/N) of the basic observable. From this quantity alone,  valuable information can be extracted; It can, for example, be used to infer the existence or absence of sources at a given redshift. As we will show below, it can also be used to probe the local properties of an unknown redshift distribution. 
%

%While somewhat less accurate than the method proposed by \citet{New:08} and recently optmized by \citet{McQ:13}, our proposed method is significantly more sensitive and can be applied to numerous datasets. From a practical point of view we also note that analyses of real-world data (for example in the optical and the infrared regimes) tend to be much less affected by systematics on small scales. Working on scales smaller than a degree (or a few projected Mpc) can be quite valuable. In this paper, we advocate for this approach and demonstrate that cluster-based redshifts provide us with a powerful exploratory tool.\\

%c
%Contrarily to the studies mentioned above, we do not aim at developing a tool as accurate as possible but instead show how useful information can be extracted from various datasets.\\
%We will show that while a trade off exists between the detectability of the cross-correlation and the accuracy of the redshift distribution estimate, useful information can be extracted from small scale clustering.


%In practice approaching this limit requires selecting a reference population within a redshift slice centered on $z$ with a narrow width $\delta z$. If one wishes to detect a non-zero cross-correlation at that redshift, this imposes a lower limit on the density of reference objects in the sky. When focusing on small angular scales, where measurements are limited by shot noise, it is given by
%\begin{equation}
%\frac{\d N_r}{\d z} >
%\frac{1}{\delta z}\,
%\frac{\pi\,\theta^2}{\langle n_u\rangle \,\bar w^2}~.
%\label{eq:detectability}
%\end{equation}
%As an example, if we consider clustering measurements on scales of 1 degree, this translates into
%\begin{equation}
%\frac{\d N_r}{\d z} \gtrsim
%%3\times
%10^3\,
%\left( \frac{0.1}{\delta z} \right) \,
%\left( \frac{100\,{\rm deg^{-2}}}{\langle n_u\ \rangle} \right) \,.
%\end{equation}
%As we will show in section \ref{sec:strategy}, various datasets satisfy this criterion. We note that the detectabi%lity condition given in Eq.~\ref{eq:detectability}  is not required for redshift inferrence. The method can be %used to generate a large number of noise-dominated cross-correlation estimates which can then be analyzed statistically. 



